Fixed-point pure gauge action using $ b= \sqrt{3} $ RGT

We present a status report on the construction of the classical perfect action using the $ b=\sqrt{3} $ renormalization group transformation (RGT). We investigate finite volume corrections and map the locality of the fixed-point action by tuning the RGT parameter, $\kappa$. We compare results with the previous calculation for b=2 RGT.

==> Makefile <==
# %auto-ignore
MAINFILE=  fp.tex
TEXFILES=  
AXISFILES= 
FIGFILES=
EPSFILES= block.eps fig.comb.fit.ps fig.comb.loc.ps fig.comb.vol.ps 

#########################################################################
# List of all the sources
SOURCES= Makefile ${MAINFILE} ${TEXFILES} ${AXISFILES} ${FIGFILES} ${EPSFILES}

# List of all postscript figures to be included.
PSINCLUSIONS= ${AXISFILES:.ax=.eps} ${FIGFILES:.fig=.eps} ${EPSFILES}

# what is to be made by default
all: ${MAINFILE:.tex=.ps}

# re-dvips if any of these change
${MAINFILE:.tex=.ps}: ${MAINFILE:.tex=.dvi} ${PSINCLUSIONS}

# re-latex if any of these change
${MAINFILE:.tex=.dvi}: ${MAIN} ${TEXFILES} ${PSINCLUSIONS}

# Never try to `make' any of the sources
${SOURCES}:;

# The rest of them do not have any `extra' dependencies, i.e. a.x depends 
# obviously depends on a.y if a.x is to be created from a.y.

.PHONY: clean realclean
# clean removes ~ aux log and tmp files
clean:
	rm -f *~ *.aux *.log *.tmp
# real clean removes everything but sources and final products
realclean: clean
	rm -f ${AXISFILES:.ax=.ps} ${AXISFILES:.ax=.eps} ${FIGFILES:.fig=.eps}

########################################################################
# General rules of how to build something from something else.
.SUFFIXES: .ps .eps .dvi .tex .ax .xy .fig

# If .fig exists that is how to create eps.
%.eps: %.fig
	fig2dev -L ps $< > $@

# else try to create it from ps
%.eps: %.ps
	sed -e "s/%%BoundingBox: 0.*/`psbbox $<`/" $< > $@ 

# If .ax or .xy exist, that is the source of the .ps file
%.ps: %.ax
	xyplot $< | epsplot > $@
%.ps: %.xy
	xyplot $< | epsplot > $@

# else look for a dvi file.
%.ps: %.dvi
	dvips -z -o $@ $<


# dvi is always created from tex.
%.dvi: %.tex
	latex $< && latex $< && latex $<

##################################################################

submission: ${SOURCES} ${PSINCLUSIONS}
	(echo "."; \
	 echo "${SOURCES} ${PSINCLUSIONS}" ; \
	 echo "submission") | uufiles -gz -9












